Discovery of fully efficient fault indicators along a data-based diagnosis process

The integration of model-based and data-driven paradigms provides a powerful framework for fault diagnosis by combining the interpretability of analytical redundancy relations, i.e., input-output relations that are used as diagnosis indicators in model-based diagnosis, with the adaptability of learning techniques. DT4X is a recent diagnosis algorithm that uses symbolic regression to generate multivariate relations leveraging some properties of analytical redundancy relations and uses them as split functions in a decision tree. However, its symbolic regression procedure optimizes only the separation between two selected classes at each node, often fragmenting the remaining classes and degrading both interpretability and diagnosis performance. This paper introduces DT4X+, an enhanced version of DT4X that modifies the construction of training sets and the symbolic-regression loss so that expressions separate the target classes while preserving the coherence of non-target classes. The resulting relations become fully consistent with ARR properties and lead to more informative splits, improved robustness, and better performance on dynamic-system datasets. Experiments conducted on several benchmark systems demonstrate the benefits of this enhanced formulation.

==> appendices.tex <==
\appendix

\begin{comment}
\section{Log loss to accuracy conversion}
\label{apdx:log_loss}
%In order to avoid applying the logarithm function to 0, the \textproc{log\_loss} function in $gplearn$ uses a technique known as clipping, which consists in replacing probabilities equal to 0 with $10^{-15}$. Given that DT4X uses \textproc{log\_loss} with a decision function that can only return 0 or 1, that meant that the \textproc{log\_loss} of a sample can only take the values \{$10^{-15}, 1-10^{-15}$\}. The total log-loss is thus a linear transformation of the number of misclassified samples. From this, we can derive:
%\[log\_loss < 1 \Leftrightarrow (1 - accuracy)\times 34.54 < 1\]
%\[\Leftrightarrow accuracy > 0.97\]
%This value corresponds to the minimum target-class separation quality required for an expression to be considered satisfactory by the DT4X fitness function.

The \textproc{log\_loss} function in \texttt{gplearn} cannot operate on probabilities equal to~0, since 
$\log(0)$ is undefined. To avoid this issue, the implementation uses \emph{clipping}, replacing 
predicted probabilities equal to~0 with $10^{-15}$, and probabilities equal to~1 with 
$1 - 10^{-15}$. In DT4X, the decision function outputs only $0$ or $1$, so after clipping, the 
effective probabilities passed to \textproc{log\_loss} are restricted to the set 
$\{10^{-15},\, 1 - 10^{-15}\}$. As a consequence, the log-loss of a sample takes only two 
possible values, depending solely on whether the sample is correctly or incorrectly classified.

For a misclassified sample, the clipped probability is $p = 10^{-15}$, leading to a log-loss of
\[
    -\log(10^{-15}) = 15 \log(10) \approx 34.54.
\]
For a correctly classified sample, the clipped probability is $p = 1 - 10^{-15}$, for which
\[
    -\log(1 - 10^{-15}) \approx 10^{-15},
\]
a negligible value. Thus, the total log-loss becomes essentially proportional to the number of 
misclassified samples. Let $N$ be the total number of samples and $N_{\text{incorrect}}$ the number of 
misclassified ones. The accuracy is defined as
\[
    \text{accuracy} = 1 - \frac{N_{\text{incorrect}}}{N}.
\]
Since each misclassified sample contributes approximately $34.54$ to the log-loss, we obtain
\[
    \text{log\_loss} \approx (1 - \text{accuracy}) \times 34.54.
\]
Hence,
\[
    \text{log\_loss} < 1
    \;\;\Leftrightarrow\;\;
    (1 - \text{accuracy}) \times 34.54 < 1
    \;\;\Leftrightarrow\;\;
    \text{accuracy} > 0.97.
\]
This threshold corresponds to the minimum target-class separation quality required for an expression
to be considered satisfactory by the DT4X fitness function.
\end{comment}

\section{Hyperparameters}
\label{apdx:hyperparam}
\begin{table}[htpb]
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{|c|c|}\hline
         \textbf{System} & \textbf{Hyperparameters} \\\hline
         sf\_polybox & \makecell[l]{
            parsimony\_coefficient=0.06, max\_depth=2,\\
            arr\_perf\_threshold=0.97, number\_of\_generations=20,\\
            population\_size=20000, function\_set=\{add, sub, mul\}} \\\hline
         sf\_subtractor & \makecell[l]{
            parsimony\_coefficient=0.05, max\_depth=2,\\
            arr\_perf\_threshold=0.97, population\_size=10000,\\
            function\_set=\{xor\_func, not\_func, or\_func, and\_func\}} \\\hline
         sw\_water\_tanks & \makecell[l]{
            epsilon=0.03, parsimony\_coefficient=0.0002, max\_depth=6,\\
            relevant\_proportion\_of\_individuals=0.0001,\\
            number\_of\_generations=35, function\_set=\{add, sub, mul,\\
            div\_custom, sqrt\_custom, sqr\_custom\}} \\\hline
         steam\_superheater\_42 & \makecell[l]{
            epsilon=0.01, parsimony\_coefficient=0.0005, max\_depth=6,\\
            relevant\_proportion\_of\_individuals=0.01,\\
            number\_of\_generations=40, population\_size=5000,\\
            function\_set=\{add, sub, mul, div\_custom\}} \\\hline
    \end{tabular}
    }
    \caption{Hyperparameters per system.}
    \label{tab:hyperparameters}
\end{table}

\section{Tree and confusion matrix comparison}
\label{apdx:tree-comparision}

As mentioned in Sec.~\ref{sec:results}, the performance metrics do not tell the whole story, with the confusion matrices and tree structures revealing extra insights into the comparison of the algorithms.

\begin{figure}[htpb]]
  \includegraphics[width=0.8\linewidth]{ifacconf_latex/images/DT4X_confusion_matrix.png}
\caption{DT4X confusion matrix on the sf\_subtractor dataset.}
\label{fig:cm_DT4X}
\end{figure}

Fig.~\ref{fig:cm_DT4X} shows that DT4X does not properly differentiate between classes 1 and 2, with a significant number of both false positives and false negatives of either class being tagged as the other. 
This changes however for DT4X+, where, as seen in Fig~\ref{fig:cm_DT4X+}, a subset of class 1 is correctly identified, with no class 1 false positives, while the predicted class 2 still contains class 1 individuals.

\begin{figure}[H]
  \includegraphics[width=0.8\linewidth]{ifacconf_latex/images/DT4X_plus_confusion_matrix.png}
\caption{DT4X+ confusion matrix on the sf\_subtractor dataset.}
\label{fig:cm_DT4X+}
\end{figure}

Furthermore, when looking at the tree structure in Fig.~\ref{fig:tree_DT4X}, we can see that the expression at Node 0 does not give any information about class 2, with its samples ending up in both Node 1 and Node 2. This is not the case with the tree generated by DT4X+ as seen in Fig.~\ref{fig:tree_DT4X+}, where no class 2 samples can be found in Node 2, meaning that the fault indicator found by DT4X+ for Node 0 is more useful than the one found by DT4X.

While the trees generated by either algorithm for the sw\_water\_tanks dataset are too large to be shown here in their entirety, Fig.~\ref{fig:DT4X_top} and Fig.~\ref{fig:DT4X+_top} show the top split of respectively, DT4X and DT4X+. On the one hand, as shown in Fig.~\ref{fig:DT4X_top}, DT4X splits most classes into both nodes only really providing information about classes 0, 1, 2 and 3, while the other classes are split among Node 1 and Node 2. On the other hand, Fig.~\ref{fig:DT4X+_top} shows that DT4X+ isolated each of the classes into one of the two nodes, with only classes 0, 3, 5 and 10 having a presence in both Node 1 and 2, though still having a very significant majority in one of the two nodes.

\begin{figure}[h]
    \centering
\tikzset{every tree node/.style={minimum width=2em,draw,rectangle},
     blank/.style={draw=none},
     edge from parent/.style=
     {draw, edge from parent path={(\tikzparentnode) -- (\tikzchildnode)}},
     level distance=6.5cm}
\resizebox{0.6\columnwidth}{!}{%
\begin{tikzpicture} 
\Tree
[.\makecell{Node : 0\\$(-d\_y4 + (y3 - y4)^4/y3)^4$\\0 vs 8\\class 0 (Faultless) : 91024 \\class 1 (f\_a) : 22553 \\class 2 (f\_hl) : 21825 \\class 3 (f\_h2) : 21715 \\class 4 (f\_f1) : 21871 \\class 5 (f\_f2) : 21100 \\class 6 (f\_11) : 20472 \\class 7 (f\_12) : 21831\\ class 8 (f\_l3) : 23535\\ class 9 (f\_cl) : 21157\\ class 10 (f\_c2) : 21005}
    [.\makecell{Node : 1\\ class 0 (Faultless) : 91020\\ class 1 (f\_a) : 22553\\ class 2 (f\_hl) : 21825\\ class 3 (f\_h2) : 21715\\ class 4 (f\_f1) : 2866\\ class 5 (f\_f2) : 8706\\ class 6 (f\_l1) : 19304\\ class 7 (f\_l2) : 791\\ class 9 (f\_c1) : 20412\\ class 10 (f\_c2) : 15791} ]
    [.\makecell{Node: 2\\ class 4 (f\_f1) : 19005\\ class 5 (f\_f2) : 12394\\class 6 (f\_l1) : 1168\\class 7 (f\_l2) : 21040\\ class 8 (f\_13) : 23535\\class 9 (f\_c1) : 745\\ class 10 (f\_c2) : 5214} ] 
]
\end{tikzpicture}
    }
    \caption{Top split of the DT4X tree for sw\_water\_tanks.}
    \label{fig:DT4X_top}
\end{figure}


\begin{figure}[h]
    \centering
\tikzset{every tree node/.style={minimum width=2em,draw,rectangle},
     blank/.style={draw=none},
     edge from parent/.style=
     {draw, edge from parent path={(\tikzparentnode) -- (\tikzchildnode)}},
     level distance=6.5cm}
\resizebox{0.8\columnwidth}{!}{%
\begin{tikzpicture} 
\Tree
[.\makecell{Node : 0\\$(d\_y2/d\_y4 + d\_y4*y4^3/y2 - y3^{0.25})/(d\_y2^2/d\_y4^2 + u\_ref + y4^6/y2^2)$\\0 vs 8\\class 0 (Faultless) : 91024 \\class 1 (f\_a) : 22553 \\class 2 (f\_h1) : 21825 \\class 3 (f\_h2) : 21715 \\class 4 (f\_f1) : 21871 \\class 5 (f\_f2) : 21100 \\class 6 (f\_l1) : 20472 \\class 7 (f\_l2) : 21831\\ class 8 (f\_l3) : 23535\\ class 9 (f\_c1) : 21157\\ class 10 (f\_c2) : 21005}
    [.\makecell{Node : 1\\ class 0 (Faultless) : 91020\\ class 1 (f\_a) : 22553\\ class 2 (f\_h1) : 21825\\ class 3 (f\_h2) : 21714\\ class 4 (f\_f1) : 21871\\ class 5 (f\_f2) : 21048\\ class 6 (f\_l1) : 20472\\ class 7 (f\_l2) : 21831\\ class 9 (f\_c1) : 21157\\ class 10 (f\_c2) : 1} ]
    [.\makecell{Node: 2\\ class 0 (Faultless) : 4\\ class 3 (f\_h2) : 1\\ class 5 (f\_f2) : 52\\ class 8 (f\_l3) : 23535\\ class 10 (f\_c2) : 21004} ] 
]
\end{tikzpicture}
    }
    \caption{Top split of the DT4X+ tree for sw\_water\_tanks.}
    \label{fig:DT4X+_top}
\end{figure}

\begin{figure*}
\centering
  \includegraphics[width=0.8\textwidth]{ifacconf_latex/images/DT4X_Tree.png}
  \caption{DT4X tree for the sf\_subtractor dataset.}
\label{fig:tree_DT4X}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{ifacconf_latex/images/DT4X_plus_Tree.png}
    \caption{DT4X+ tree for the sf\_subtractor dataset.}
    \label{fig:tree_DT4X+}
\end{figure*}
